Novel View Synthesis of Humans using Differentiable Rendering

We present a new approach for synthesizing novel views of people in new poses. Our novel differentiable renderer enables the synthesis of highly realistic images from any viewpoint. Rather than operating over mesh-based structures, our renderer makes use of diffuse Gaussian primitives that directly represent the underlying skeletal structure of a human. Rendering these primitives gives results in a high-dimensional latent image, which is then transformed into an RGB image by a decoder network. The formulation gives rise to a fully differentiable framework that can be trained end-to-end. We demonstrate the effectiveness of our approach to image reconstruction on both the Human3.6M and Panoptic Studio datasets. We show how our approach can be used for motion transfer between individuals; novel view synthesis of individuals captured from just a single camera; to synthesize individuals from any virtual viewpoint; and to re-render people in novel poses. Code and video results are available at https://github.com/GuillaumeRochette/HumanViewSynthesis.

==> latexmkrc <==
# Settings
$xdvipdfmx = "xdvipdfmx -z 6 -o %D %O %S";

###############################
# Post processing of pdf file #
###############################

# assume the jobname is 'output' for sharelatex
my $ORIG_PDF_AGE = -M "output.pdf"; # get age of existing pdf if present

END {
    my $NEW_PDF_AGE = -M "output.pdf";
    return if !defined($NEW_PDF_AGE); # bail out if no pdf file
    return if defined($ORIG_PDF_AGE) && $NEW_PDF_AGE == $ORIG_PDF_AGE; # bail out if pdf was not updated
    $qpdf //= "/usr/local/bin/qpdf";
    $qpdf = $ENV{QPDF} if defined($ENV{QPDF}) && -x $ENV{QPDF};
    return if ! -x $qpdf; # check that qpdf exists
    $qpdf_opts //= "--linearize --newline-before-endstream";
    $qpdf_opts = $ENV{QPDF_OPTS} if defined($ENV{QPDF_OPTS});
    my $status = system($qpdf, split(' ', $qpdf_opts), "output.pdf", "output.pdf.opt");
    my $exitcode = ($status >> 8);
    print "qpdf exit code=$exitcode\n";
    # qpdf returns 0 for success, 3 for warnings (output pdf still created)
    return if !($exitcode == 0 || $exitcode == 3);
    print "Renaming optimised file to output.pdf\n";
    rename("output.pdf.opt", "output.pdf");
}

##############
# Glossaries #
##############
add_cus_dep( 'glo', 'gls', 0, 'glo2gls' );
add_cus_dep( 'acn', 'acr', 0, 'glo2gls');  # from Overleaf v1
sub glo2gls {
    system("makeglossaries $_[0]");
}

#############
# makeindex #
#############
@ist = glob("*.ist");
if (scalar(@ist) > 0) {
    $makeindex = "makeindex -s $ist[0] %O -o %D %S";
}

################
# nomenclature #
################
add_cus_dep("nlo", "nls", 0, "nlo2nls");
sub nlo2nls {
        system("makeindex $_[0].nlo -s nomencl.ist -o $_[0].nls -t $_[0].nlg");
}

#########
# Knitr #
#########
my $root_file = $ARGV[-1];

add_cus_dep( 'Rtex', 'tex', 0, 'rtex_to_tex');
sub rtex_to_tex {
    do_knitr("$_[0].Rtex");
}

sub do_knitr {
    my $dirname = dirname $_[0];
    my $basename = basename $_[0];
    system("Rscript -e \"library('knitr'); setwd('$dirname'); knit('$basename')\"");
}

my $rtex_file = $root_file =~ s/\.tex$/.Rtex/r;
unless (-e $root_file) {
    if (-e $rtex_file) {
        do_knitr($rtex_file);
    }
}

##########
# feynmf #
##########
push(@file_not_found, '^feynmf: Files .* and (.*) not found:$');
add_cus_dep("mf", "tfm", 0, "mf_to_tfm");
sub mf_to_tfm { system("mf '\\mode:=laserjet; input $_[0]'"); }

push(@file_not_found, '^feynmf: Label file (.*) not found:$');
add_cus_dep("mf", "t1", 0, "mf_to_label1");
sub mf_to_label1 { system("mf '\\mode:=laserjet; input $_[0]' && touch $_[0].t1"); }
add_cus_dep("mf", "t2", 0, "mf_to_label2");
sub mf_to_label2 { system("mf '\\mode:=laserjet; input $_[0]' && touch $_[0].t2"); }
add_cus_dep("mf", "t3", 0, "mf_to_label3");
sub mf_to_label3 { system("mf '\\mode:=laserjet; input $_[0]' && touch $_[0].t3"); }
add_cus_dep("mf", "t4", 0, "mf_to_label4");
sub mf_to_label4 { system("mf '\\mode:=laserjet; input $_[0]' && touch $_[0].t4"); }
add_cus_dep("mf", "t5", 0, "mf_to_label5");
sub mf_to_label5 { system("mf '\\mode:=laserjet; input $_[0]' && touch $_[0].t5"); }
add_cus_dep("mf", "t6", 0, "mf_to_label6");
sub mf_to_label6 { system("mf '\\mode:=laserjet; input $_[0]' && touch $_[0].t6"); }
add_cus_dep("mf", "t7", 0, "mf_to_label7");
sub mf_to_label7 { system("mf '\\mode:=laserjet; input $_[0]' && touch $_[0].t7"); }
add_cus_dep("mf", "t8", 0, "mf_to_label8");
sub mf_to_label8 { system("mf '\\mode:=laserjet; input $_[0]' && touch $_[0].t8"); }
add_cus_dep("mf", "t9", 0, "mf_to_label9");
sub mf_to_label9 { system("mf '\\mode:=laserjet; input $_[0]' && touch $_[0].t9"); }

##########
# feynmp #
##########
push(@file_not_found, '^dvipdf: Could not find figure file (.*); continuing.$');
add_cus_dep("mp", "1", 0, "mp_to_eps");
sub mp_to_eps {
    system("mpost $_[0]");
    return 0;
}

#############
# asymptote #
#############
sub asy {return system("asy --offscreen '$_[0]'");}
add_cus_dep("asy","eps",0,"asy");
add_cus_dep("asy","pdf",0,"asy");
add_cus_dep("asy","tex",0,"asy");

#############
# metapost  #  # from Overleaf v1
#############
add_cus_dep('mp', '1', 0, 'mpost');
sub mpost {
    my $file = $_[0];
    my ($name, $path) = fileparse($file);
    pushd($path);
    my $return = system "mpost $name";
    popd();
    return $return;
}

##########
# chktex #
##########
unlink 'output.chktex' if -f 'output.chktex';
if (defined $ENV{'CHKTEX_OPTIONS'}) {
    use File::Basename;
    use Cwd;

    # identify the main file
    my $target = $ARGV[-1];
    my $file = basename($target);

    if ($file =~ /\.tex$/) {
        # change directory for a limited scope
        my $orig_dir = cwd();
        my $subdir = dirname($target);
        chdir($subdir);
        # run chktex on main file
        $status = system("/usr/bin/run-chktex.sh", $orig_dir, $file);
        # go back to original directory
        chdir($orig_dir);

        # in VALIDATE mode we always exit after running chktex
        # otherwise we exit if EXIT_ON_ERROR is set

        if ($ENV{'CHKTEX_EXIT_ON_ERROR'} || $ENV{'CHKTEX_VALIDATE'}) {
            # chktex doesn't let us access the error info via exit status
            # so look through the output
            open(my $fh, "<", "output.chktex");
            my $errors = 0;
            {
                local $/ = "\n";
                while(<$fh>) {
                    if (/^\S+:\d+:\d+: Error:/) {
                        $errors++;
                        print;
                    }
                }
            }
            close($fh);
            exit(1) if $errors > 0;
            exit(0) if $ENV{'CHKTEX_VALIDATE'};
        }
    }
}

add_cus_dep( 'tex', 'aux', 0, 'makeexternaldocument' );

sub makeexternaldocument {
    if (!($root_filename eq $_[0]))
    {
        system( "latexmk -cd -pdf \"$_[0]\"" );
    }
}

==> sections/commands.tex <==
\makeatletter
\newcommand*{\addFileDependency}[1]{
  \typeout{(#1)}
  \@addtofilelist{#1}
  \IfFileExists{#1}{}{\typeout{No file #1.}}
}
\makeatother

\newcommand*{\myexternaldocument}[1]{%
    \externaldocument{#1}%
    \addFileDependency{#1.tex}%
    \addFileDependency{#1.aux}%
}

\makeatletter
\DeclareRobustCommand\onedot{\futurelet\@let@token\@onedot}
\def\@onedot{\ifx\@let@token.\else.\null\fi\xspace}
\def\eg{\emph{e.g}\onedot} \def\Eg{\emph{E.g}\onedot}
\def\ie{\emph{i.e}\onedot} \def\Ie{\emph{I.e}\onedot}
\def\cf{\emph{c.f}\onedot} \def\Cf{\emph{C.f}\onedot}
\def\etc{\emph{etc}\onedot} \def\vs{\emph{vs}\onedot}
\def\wrt{w.r.t\onedot} \def\dof{d.o.f\onedot}
\def\etal{\emph{et al}\onedot}
\makeatother

\newcommand*{\sbf}[3]{{#1}^\intercal {#2}^{-1} {#3}}
\newcommand*{\argmin}{\operatornamewithlimits{argmin}}
\newcommand*{\argmax}{\operatornamewithlimits{argmax}}
\newcommand*{\erf}{\operatornamewithlimits{erf}}
\newcommand*{\erfc}{\operatornamewithlimits{erfc}}


==> tables/fused_inference.tex <==
\begin{table}[tbp]
    \centering
    \caption{Evolution of the PSNR, SSIM, LPIPS, and MPJPE against the number of input views.}
    \resizebox{\linewidth}{!}{%
    \begin{tabular}{@{}lccccccc@{}}
    \toprule
    No. of Views & $\text{MPJPE}_{\text{B}}$ $\downarrow$  & $\text{MPJPE}_{\text{L}}$ $\downarrow$ & $\text{MPJPE}_{\text{R}}$ $\downarrow$ & $\text{MPJPE}_{\text{F}}$ $\downarrow$ & LPIPS $\downarrow$ & PSNR $\uparrow$  & SSIM $\uparrow$  \\
    \midrule
    1             & 20.83 & 14.59      & 14.36       & 3.67 & 0.0323 & 31.13 & 0.9521 \\
    2             & 19.00 & 13.48      & 13.37       & 3.46 & 0.0307 & 31.43 & 0.9534 \\
    3             & 18.16 & 13.18      & 12.92       & 3.38 & 0.0300 & 31.58 & 0.9540 \\
    4             & 17.49 & 12.83      & 12.63       & 3.32 & 0.0294 & 31.70 & 0.9545 \\
    5             & 17.05 & 12.54      & 12.40       & 3.28 & 0.0291 & 31.79 & 0.9549 \\
    6             & 16.75 & 12.33      & 12.20       & 3.25 & 0.0288 & 31.84 & 0.9551 \\
    7             & 16.49 & 12.18      & 12.07       & 3.22 & 0.0286 & 31.89 & 0.9553 \\
    8             & 16.29 & 12.08      & 11.95       & 3.20 & 0.0284 & 31.93 & 0.9554 \\
    9             & 16.12 & 11.94      & 11.85       & 3.19 & 0.0282 & 31.96 & 0.9556 \\
    10            & 16.00 & 11.84      & 11.75       & 3.17 & 0.0281 & 31.99 & 0.9557 \\
    11            & 15.88 & 11.78      & 11.70       & 3.16 & 0.0280 & 32.01 & 0.9558 \\
    12            & 15.77 & 11.71      & 11.60       & 3.15 & 0.0279 & 32.03 & 0.9558 \\
    13            & 15.68 & 11.66      & 11.56       & 3.14 & 0.0279 & 32.04 & 0.9559 \\
    14            & 15.62 & 11.60      & 11.53       & 3.13 & 0.0278 & 32.05 & 0.9559 \\
    15            & 15.54 & 11.51      & 11.47       & 3.12 & 0.0277 & 32.07 & 0.9560 \\
    16            & 15.48 & 11.48      & 11.42       & 3.12 & 0.0277 & 32.08 & 0.9560 \\
    17            & 15.42 & 11.45      & 11.39       & 3.11 & 0.0276 & 32.09 & 0.9561 \\
    18            & 15.39 & 11.41      & 11.36       & 3.11 & 0.0276 & 32.10 & 0.9561 \\
    19            & 15.35 & 11.38      & 11.34       & 3.10 & 0.0276 & 32.11 & 0.9561 \\
    20            & 15.31 & 11.35      & 11.31       & 3.10 & 0.0275 & 32.11 & 0.9562 \\
    21            & 15.27 & 11.32      & 11.29       & 3.10 & 0.0275 & 32.12 & 0.9562 \\
    22            & 15.23 & 11.31      & 11.28       & 3.09 & 0.0275 & 32.13 & 0.9562 \\
    23            & 15.21 & 11.29      & 11.28       & 3.09 & 0.0275 & 32.13 & 0.9562 \\
    24            & 15.18 & 11.28      & 11.27       & 3.09 & 0.0274 & 32.14 & 0.9563 \\
    25            & 15.15 & 11.27      & 11.25       & 3.08 & 0.0274 & 32.14 & 0.9563 \\
    \bottomrule
    \end{tabular}%
    }
    \label{tab:FusedInferencePanoptic}
\end{table}

\begin{table}[tbp]
    \centering
    \caption{Evolution of the PSNR, SSIM, LPIPS, and MPJPE against the number of input views.}
    \resizebox{\linewidth}{!} {%
    \begin{tabular}{@{}lcccccc@{}}
    \toprule
    No. of Views & MPJPE $\downarrow$ & NMPJPE $\downarrow$ & PMJPE $\downarrow$ & LPIPS $\downarrow$  & PSNR $\uparrow$  & SSIM $\uparrow$   \\
    \midrule
    1            & 36.76 & 36.20  & 30.51 & 0.0792 & 21.17 & 0.8669 \\
    2            & 31.45 & 30.91  & 26.27 & 0.0724 & 21.64 & 0.8739 \\
    3            & 29.31 & 28.79  & 24.53 & 0.0696 & 21.92 & 0.8778 \\
    4            & 28.32 & 27.78  & 23.68 & 0.0682 & 22.04 & 0.8795 \\
    \bottomrule
    \end{tabular}%
    }
    \label{tab:FusedInferenceHuman36M}
\end{table}

